Gaussian Splatting in Style

3D scene stylization extends the work of neural style transfer to 3D. A vital challenge in this problem is to maintain the uniformity of the stylized appearance across multiple views. A vast majority of the previous works achieve this by training a 3D model for every stylized image and a set of multi-view images. In contrast, we propose a novel architecture trained on a collection of style images that, at test time, produces real time high-quality stylized novel views. We choose the underlying 3D scene representation for our model as 3D Gaussian splatting. We take the 3D Gaussians and process them using a multi-resolution hash grid and a tiny MLP to obtain stylized views. The MLP is conditioned on different style codes for generalization to different styles during test time. The explicit nature of 3D Gaussians gives us inherent advantages over NeRF-based methods, including geometric consistency and a fast training and rendering regime. This enables our method to be useful for various practical use cases, such as augmented or virtual reality. We demonstrate that our method achieves state-of-the-art performance with superior visual quality on various indoor and outdoor real-world data.

==> tables/consistency-brief.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{|c|c|c|ccccccc|}
\hline
Dataset ↓ &
  \begin{tabular}[c]{@{}c@{}}Consis-\\ tency ↓\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Metric ↓ \\ Method→\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}GS → \\ AdaIN\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdaIN → \\ GS\end{tabular}} &
  \multicolumn{1}{c|}{LSNV} &
  \multicolumn{1}{c|}{ARF} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Stylised-\\ NeRF\end{tabular}} &
  \multicolumn{1}{c|}{StyleRF} &
  Ours \\ \hline
                       &                              & RMSE  & 0.122 & 0.106 & 0.069 & 0.039 & \cellcolor[HTML]{FFFFC7}0.028 & 0.039 & \cellcolor[HTML]{9AFF99}0.019 \\ \cline{3-10} 
                       & \multirow{-2}{*}{Short-Term} & LPIPS & 0.132 & 0.109 & 0.032 & 0.019 & \cellcolor[HTML]{FFFFC7}0.009 & 0.017 & \cellcolor[HTML]{9AFF99}0.005 \\ \cline{2-10} 
                       &                              & RMSE  & 0.153 & 0.138 & 0.070 & 0.095 & \cellcolor[HTML]{FFFFC7}0.040 & 0.095 & \cellcolor[HTML]{9AFF99}0.032 \\ \cline{3-10} 
\multirow{-4}{*}{LLFF} & \multirow{-2}{*}{Long-Term}  & LPIPS & 0.190 & 0.161 & 0.040 & 0.083 & \cellcolor[HTML]{FFFFC7}0.021 & 0.067 & \cellcolor[HTML]{9AFF99}0.014 \\ \hline
                       &                              & RMSE  & 0.116 & 0.100 & 0.059 & 0.038 & 0.022                         & 0.039 & 0.023                         \\ \cline{3-10} 
                       & \multirow{-2}{*}{Short-Term} & LPIPS & 0.126 & 0.101 & 0.027 & 0.018 & 0.007                         & 0.016 & 0.006                         \\ \cline{2-10} 
                       &                              & RMSE  & 0.151 & 0.138 & 0.063 & 0.102 & 0.030                         & 0.102 & 0.046                         \\ \cline{3-10} 
\multirow{-4}{*}{TnT}  & \multirow{-2}{*}{Long-Term}  & LPIPS & 0.180 & 0.155 & 0.034 & 0.090 & 0.016                         & 0.070 & 0.025                         \\ \hline
\end{tabular}
\end{table}

==> tables/long_term_full.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|ccccccc|}
\hline
\begin{tabular}[c]{@{}c@{}}Dataset\\ ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Method\\ →\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}GS → \\ AdaIN\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdaIN \\ → GS\end{tabular}} & \multicolumn{1}{c|}{LSNV}     & \multicolumn{1}{c|}{ARF} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Stylised-\\ NeRF\end{tabular}} & \multicolumn{1}{c|}{StyleRF} & GSS(Ours)                     \\ \hline
                                                    & RMSE ↓                                               & 0.147                                                                      & 0.141                                                                      & \cellcolor[HTML]{FFFFC7}0.040 & 0.123                    & \cellcolor[HTML]{9AFF99}0.002                                                 & 0.123                        & 0.090                         \\
\multirow{-2}{*}{Flower}                            & LPIPS ↓                                              & 0.151                                                                      & 0.135                                                                      & 0.018                         & 0.112                    & \cellcolor[HTML]{9AFF99}0.001                                                 & 0.081                        & \cellcolor[HTML]{FFFFC7}0.057 \\ \hline
                                                    & RMSE ↓                                               & 0.151                                                                      & 0.132                                                                      & 0.076                         & 0.109                    & \cellcolor[HTML]{FFFFC7}0.044                                                 & 0.115                        & \cellcolor[HTML]{9AFF99}0.042 \\
\multirow{-2}{*}{Fern}                              & LPIPS ↓                                              & 0.193                                                                      & 0.162                                                                      & 0.051                         & 0.107                    & \cellcolor[HTML]{FFFFC7}0.019                                                 & 0.099                        & \cellcolor[HTML]{9AFF99}0.021 \\ \hline
                                                    & RMSE ↓                                               & 0.143                                                                      & 0.150                                                                      & \cellcolor[HTML]{FFFFC7}0.045 & 0.084                    & \cellcolor[HTML]{FFFFC7}0.045                                                 & 0.078                        & \cellcolor[HTML]{9AFF99}0.033 \\
\multirow{-2}{*}{Room}                              & LPIPS ↓                                              & 0.182                                                                      & 0.184                                                                      & 0.019                         & 0.061                    & \cellcolor[HTML]{FFFFC7}0.028                                                 & 0.046                        & \cellcolor[HTML]{9AFF99}0.015 \\ \cline{1-8}
                                                    & RMSE ↓                                               & 0.164                                                                      & 0.131                                                                      & 0.091                         & 0.092                    & \cellcolor[HTML]{FFFFC7}0.030                                                 & 0.091                        & \cellcolor[HTML]{9AFF99}0.020 \\
\multirow{-2}{*}{Trex}                              & LPIPS ↓                                              & 0.194                                                                      & 0.137                                                                      & 0.050                         & 0.081                    & \cellcolor[HTML]{FFFFC7}0.016                                                 & 0.057                        & \cellcolor[HTML]{9AFF99}0.007 \\ \hline
\end{tabular}
\caption{\textbf{Long Term Consistency} In this table, we measure the performance of GSS against the said baselines via long-term consistency. Similar to \cite{liu2023stylerf}, for long-term consistency, the two frames should be far away from each other. Having a long-term consistent method ensures that the produced novel views of the scene are consistent in the stylized color space. Similar to short-term consistency in \Cref{table:short_term}, StylizedNerf numbers does not accurately depict the stylization quality as compared to other methods.}
\label{table:long_term}
\vspace{-2cm}
\end{table}

==> tables/short_term_full.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{|c|c|ccccccc|}
\hline
\begin{tabular}[c]{@{}c@{}}Dataset\\ ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Method\\ →\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}GS →   \\ AdaIN\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdaIN   \\ → GS\end{tabular}} & \multicolumn{1}{c|}{LSNV}     & \multicolumn{1}{c|}{ARF} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Stylised-  \\ NeRF\end{tabular}} & \multicolumn{1}{c|}{StyleRF}  & GSS(Ours)                     \\ \hline
                                                    & RMSE ↓                                               & 0.098                                                                        & 0.083                                                                        & \cellcolor[HTML]{FFFFC7}0.030 & 0.036                    & \cellcolor[HTML]{9AFF99}0.002                                                   & 0.038                         & 0.034                         \\ \cline{2-2}
\multirow{-2}{*}{Flower}                            & LPIPS ↓                                              & 0.106                                                                        & 0.080                                                                        & 0.011                         & 0.015                    & \cellcolor[HTML]{9AFF99}0.001                                                   & 0.013                         & \cellcolor[HTML]{FFFFC7}0.009 \\ \hline
                                                    & RMSE ↓                                               & 0.127                                                                        & 0.116                                                                        & 0.075                         & 0.038                    & 0.041                                                                           & \cellcolor[HTML]{FFFFC7}0.037 & \cellcolor[HTML]{9AFF99}0.026 \\
\multirow{-2}{*}{Fern}                              & LPIPS ↓                                              & 0.151                                                                        & 0.134                                                                        & 0.049                         & 0.020                    & \cellcolor[HTML]{FFFFC7}0.012                                                   & 0.019                         & \cellcolor[HTML]{9AFF99}0.008 \\ \hline
                                                    & RMSE ↓                                               & 0.104                                                                        & 0.103                                                                        & 0.044                         & 0.037                    & \cellcolor[HTML]{FFFFC7}0.029                                                   & 0.035                         & \cellcolor[HTML]{9AFF99}0.021 \\
\multirow{-2}{*}{Room}                              & LPIPS ↓                                              & 0.109                                                                        & 0.105                                                                        & 0.014                         & 0.014                    & \cellcolor[HTML]{FFFFC7}0.011                                                   & 0.014                         & \cellcolor[HTML]{9AFF99}0.006 \\ \hline
                                                    & RMSE ↓                                               & 0.136                                                                        & 0.099                                                                        & 0.089                         & 0.043                    & \cellcolor[HTML]{FFFFC7}0.015                                                   & 0.045                         & \cellcolor[HTML]{9AFF99}0.010 \\
\multirow{-2}{*}{Trex}                              & LPIPS ↓                                              & 0.136                                                                        & 0.087                                                                        & 0.033                         & 0.022                    & \cellcolor[HTML]{FFFFC7}0.004                                                   & 0.017                         & \cellcolor[HTML]{9AFF99}0.003 \\ \hline
\end{tabular}
\caption{\textbf{Short Term Consistency} Here, we demonstrate the superior performance of our method using the short-term consistency metric. We compute the metric using both, RMSE and LPIPS\cite{zhang2018perceptual} using a VGG backbone. As shown in \Cref{fig:qual_result}, the novel views rendered by StylizedNerf are highly blurry and misses crucial details. Therefore, due to the over-smooth and blurry output, the metric obtained for them is really low and does not correctly reflect the adequate stylization qualities. }
\label{table:short_term}
\vspace{-1cm}
\end{table}
